When and Why Momentum Accelerates SGD:An Empirical Study

Momentum has become a crucial component in deep learning optimizers, necessitating a comprehensive understanding of when and why it accelerates stochastic gradient descent (SGD). To address the question of ''when'', we establish a meaningful comparison framework that examines the performance of SGD with Momentum (SGDM) under the \emph{effective learning rates} $\eta_{ef}$, a notion unifying the influence of momentum coefficient $\mu$ and batch size $b$ over learning rate $\eta$. In the comparison of SGDM and SGD with the same effective learning rate and the same batch size, we observe a consistent pattern: when $\eta_{ef}$ is small, SGDM and SGD experience almost the same empirical training losses; when $\eta_{ef}$ surpasses a certain threshold, SGDM begins to perform better than SGD. Furthermore, we observe that the advantage of SGDM over SGD becomes more pronounced with a larger batch size. For the question of ``why'', we find that the momentum acceleration is closely related to \emph{abrupt sharpening} which is to describe a sudden jump of the directional Hessian along the update direction. Specifically, the misalignment between SGD and SGDM happens at the same moment that SGD experiences abrupt sharpening and converges slower. Momentum improves the performance of SGDM by preventing or deferring the occurrence of abrupt sharpening. Together, this study unveils the interplay between momentum, learning rates, and batch sizes, thus improving our understanding of momentum acceleration.

==> Tex_files/Preliminary.tex <==
\section{Preliminary}

 First-order optimizers are frequently applied to resolve such problems, with the most basic one being the stochastic gradient descent (SGD) optimizer. The corresponding update rule for SGD is:
\begin{equation*}
    \bw_{t+1}=\bw_t -\eta_t \nabla  f_{\xi_t}(\bw_t),
\end{equation*}
where $\nabla f_{\xi_t}(\bw_t)$ is the stochastic estimate of the gradient of $f$ at $\bw_t$, and $\xi_t$ a random variable. Despite the simple form of SGD, its training speed is not satisfactory over many deep learning tasks. To overcome this challenge,  stochastic gradient descent with momentum is proposed, which replace the single gradient of current iteration in SGD by a weighted average of historical gradients (called "momentum"\citep{sutskever2013importance}): 
\begin{gather}
\nonumber
\bom_{t}=\mu \bom_{t-1}+\nabla  f_{\xi_t}(\bw_{t}), 
\\
\label{def: sgdm}
    \bw_{t+1}=\bw_{t} - \eta_t \bom_{t}.
\end{gather}
 When $\mu=0$, SGDM degenerates to SGD.

We define the effective learning rate as:
\begin{equation*}
    \eta_{\ef}=\underbrace{\frac{1}{1-\mu}}_{\text{effect of momentum}} \overbrace{\frac{K}{B}}^{\text{Linear Scaling Rule}} \eta,
\end{equation*}
where $B$ denotes the batch size.
Our goal with the effective learning rate is to harmonize the learning rate settings for various momentum coefficients ($\mu$) and batch sizes. To align different momentum coefficients, we utilize the factor $\frac{1}{1-\mu}$. Additionally, we employ the Linear Scaling Rule\cite{goyal2017accurate} to align the training for different batch sizes. $K$ is a predefined value for scaling the effective learning rate to a suitable level. If $K=B$, we obtain $\eta^{B}_{\ef}=\frac{1}{1-\mu} \eta$. \textbf{To make the notation simpler, if the value of $K$ is not explicitly set, it is assumed to be $B$ by default, meaning $\eta_{\ef}=\frac{1}{1-\mu}\eta$.}

==> Tex_files/why-bak.tex <==
\section{Why does momentum accelerate SGD?}
In Section \ref{sec:when}, we have explored when momentum accelerates SGD. In this section, we aim to study the intrinsic mechanism of the observations made in Section \ref{sec:when}. We first investigate in the full-batch case and study why momentum accelerate GD. This scenario is particularly significant because according to Figure \ref{fig:phase_transition}, 
 momentum is more effective  when a larger batch size is employed. Moreover, the full-batch update gets rid of the random noise and simplifies the analysis. As the full-batch update is computationally expansive, we focus instead on a dataset with fewer samples: we train fc-tanh\cite{cohen2021gradient} over the  Cifar10-5k dataset using GD and GDM. Note that this task has been used in \cite{cohen2021gradient,ahn2022understanding} to study the training behavior of GD. We first verify that the align-and-deviation pattern still exist in this task in Figure \ref{fig:gd}A. We then pick one effective learning rate $\eta_{\ef}=0.01$ before the deviation threshold  and one effective learning rate $\eta_{\ef}=0.1$ after the threshold and plot its training loss across epochs in Figure \ref{fig:gd}B and Figure \ref{fig:gd}C. We find:  
\begin{itemize}
    \item \textbf{The deviation between GD and GDM during training occurs concurrently as GD starts oscillating.} Before the deviation threshold ($\eta_{\ef}=0.01$), the training curves of GDM and GD are smooth and they are closely aligned (Figure \ref{fig:gd}B).  After the  deviation threshold ($\eta_{\ef}=0.1$), the training curves of GDM and GD are still smooth and aligned before GD starts oscillating. However, they diverges and GD converges slower than GDM after GD starts oscillating  (Figure \ref{fig:gd}C). In other words, momentum prevents (or defer) oscillation and accelerates GD.
\end{itemize}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7 \textwidth]{images/gdloss.png}
    \caption{\textbf{Exploration of the training process on CIFAR10-5k dataset.} A: Experiments on Cifar10-5k  gives a similar result as Figure \ref{fig:phase_transition}. B: GD and GDM are aligned during the whole training process under small learning rate. C: GD and GDM are aligned before GD starting oscillating, and deviate after. The red dash line denotes the time when the GD starts oscillating.}
    \label{fig:gd}
\end{figure}

% Then, in Section \ref{subsec:momentum_abrupt_sharpening}, we find that momentum can prevent abrupt sharpening of directional Hessian so as to defer the momentum for optimizer for enter EoS. This phenomenon can explain why Momentum can accelerate training. 
% \subsection{Revisit existing conclusion}
% \textbf{Conclusion II:} Momentum can accelerate SGD by inter playing with the noise. \cite{defazio2020momentum} gives a theoretical explaination that the momentum can reduce the noise in SGD, and as a result, make the update more close to the full batch gradient. \cite{kidambi2018insufficiency} gives a proof in toy case where the MSGD can't outperform SGD and experiments on more complicate case demonstrating that momentum helps more in small batch size setting which has higher noise level in gradient estimation.

%  \textbf{Conclusion II} can't explain why the momentum accelerate gradient descent(Figure \ref{fig:cifar10-5k}), where no noise exsits. By analyzing the case of gradient descent, we argue that it is EoS phenomenon, not the noise that cases the gap between GD and GDM.  

% \textbf{Conclusion II} SGDM can't out perform SGD  despite the best setting of its parameters.
\subsection{Abrupt Sharpening and edge of stability}
\label{subsc:eos_phasetransition}
% Section \ref{sec:when} finds a align-divergence pattern, that there is a divergence point (detail in Figure \ref{fig:phase_transition}), which distinguishes between the region where SGDM and SGD exhibit similar performance and the region where SGDM surpasses SGD. Here, we give a more detail investigation of this pattern in the full-batch scenario (i.e., we study GD and GDM). In Figure  We plot  Specifically, we would like to answer two questions:
%  \begin{enumerate}
%      \item Why GD and GDM are aligned before the divergent point?
%      \item Why GDM outperforms the GD after the divergence point?
%  \end{enumerate}
 % We first give experimental exploration for the training process with effective learning rate before and after the divergence point. 
The observation in Figure \ref{fig:gd} provides a partial answer of why momentum accelerates GD by connecting it with preventing oscillation. However, we are still unclear the reason for why the oscillations happen and why GDM is less like to oscillate. With $\bw_t$ be the iteration of GD, we revisit the Taylor expansion of the objective function $f$, which writes
\begin{equation*}
    f(\bw_{t+1})\approx f(\bw_{t})-\eta \Vert  \nabla f(\bw_t)\Vert^2 +\frac{\eta^2}{2} \nabla f(\bw_t)^{\top}\nabla^2 f(\bw_t) \nabla f(\bw_t). 
\end{equation*}
When the loss stably decreases, we have $f(\bw_{t+1})< f(\bw_{t})$, and based on the above approximation, we infer $\frac{\eta(\bw_{t+1}-\bw_t)^{\top}\nabla^2 f(\bw_t) (\bw_{t+1}-\bw_t)}{2 \Vert \bw_{t+1}-\bw_t\Vert^2}=\frac{\eta\nabla f(\bw_t)^{\top}\nabla^2 f(\bw_t) \nabla f(\bw_t)}{2 \Vert \nabla f(\bw_t)\Vert^2}< 1$. On the other hand, we have $f(\bw_{t+1})\approx f(\bw_{t})$ when oscillating \cite{ahn2022understanding}, and thus $\frac{\eta(\bw_{t+1}-\bw_t)^{\top}\nabla^2 f(\bw_t) (\bw_{t+1}-\bw_t)}{2 \Vert \bw_{t+1}-\bw_t\Vert^2}\approx 1$. Therefore, we conjecture that there is a transition of the directional Hessian $H(\bw_t,\bw_{t+1}-\bw_t)\triangleq \frac{(\bw_{t+1}-\bw_t)^{\top}\nabla^2 f(\bw_t) (\bw_{t+1}-\bw_t)}{ \Vert \bw_{t+1}-\bw_t\Vert^2}$ which leads to oscillation. We plot the directional Hessian  in Figure \ref{fig:gdhess}.  Our observation is as follows:
\begin{itemize}
    \item \textbf{Direction Hessian exhibits an "abrupt sharpening" phenomenon.} There is a clear transition of the directional Hessian: the directional Hessian  first stays around $0$ before oscillation, and then exhibits an emergent jump (referred as "abrupt sharpening") when oscillation.
\end{itemize}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95 \textwidth]{images/gdhess.png}
    \caption{\textbf{Sharpness and directional Hessian on CIFAR10-5k dataset.} The dashed blue line represents the threshold  $\frac{2}{\eta_{\ef}}$.  \textit{Left:} With a small effective learning rate, the directional Hessian of GD and GDM are around $0$.  \textit{Center:} With a larger effective learning rate, GD exhibits abrupt sharpening and training loss starts to oscillate (marked by the red dash line) when the sharpness of GD surpasses $\frac{2}{\eta_{\ef}}$, while directional Hessian of GDM stays around $0$. \textit{Right:} With an even larger effective learning rate, both GDM and GD exhibits abrupt sharpening, while GDM is much latter.}
    \label{fig:gdhess}
\end{figure}
Abrupt sharpening explains why the oscillations happen.  We further notice that abrupt sharpening is closely related to a existing concept called "edge of stability" (EoS), which describe the phenomenon that during the training of GD, sharpness (\ieno the maximum eigenvalue of Hessian) will gradually increase until it reaches $\frac{2}{\eta}$ and then hover at it. The gradually increasing behavior of sharpness is denoted as "progressive sharpening", which seems to be sharply different from abrupt sharpening, but we show through the following proposition that abrupt sharpening is a joint outcome of progressive sharpening and renowned degenerate Hessian of deep neural networks \cite{sagun2016eigenvalues}, and thus abrupt sharpening can be viewed as a newfound component of EoS.
\begin{proposition}
\label{prop: convergence_direction}
Given a minimization problem $\min_{\bw\in \mathbb{R}^d} f(\bw)$, we consider its quadratic function approximation $\tilde{f}(\bw)$ around a minimizer $\bw^*$, i.e., $\min_{\bw\in \mathbb{R}^d}$ $ \frac{1}{2}(\bw-\bw^*)^{\top} \nabla^2f(\bw^*) (\bw-\bw^*)+f(\bw^*)$. Let $\bw_t$ be the parameter given by GD at the $t$-th iteration. Let $\mathcal{A}$ be the space of eigenvectors of $\nabla^2f(\bw^*)$ corresponding to the maximum eigenvalue of $\bA$. For almost everywhere $\bw_0\in \mathbb{R}^d$ , $\lim_{t\rightarrow \infty}\frac{\nabla \tilde{f}(\bw_t)}{\Vert \nabla \tilde{f}(\bw_t) \Vert} \in \mathcal{A} $ if and only if $\lambda_{\max}(\nabla^2f(\bw^*))> \frac{2}{\eta_{\ef}}-\lambda_{\min} (\nabla^2f(\bw^*))$.
\end{proposition}
\citet{sagun2016eigenvalues} observes that in deep learning tasks, the smallest eigenvalue of Hessian $\lambda_{\min} (\nabla^2f(\bw^*))$ is close to $0$. This together with Proposition \ref{prop: convergence_direction} indicates that the update direction of GD would start to align with the eigenspace of the maximum eigenvalue only after the sharpness is very close to $\frac{2}{\eta}$ (thus in the early stage, directional sharpness stays around $0$). Once such an alignment starts, it is rapid because the convergence rate in Proposition \ref{prop: convergence_direction} is exponential (which explains the abrupt increase).


\subsection{Abrupt sharpening can explain the acceleration effect of momentum}
\label{sec: abrupt_effect}
Here we show that abrupt sharpening can be used to explain the acceleration effect of momentum.

\textbf{Small directional Hessian explains the alignment between GD and GDM.} Intuitively, when directional Hessian is relatively small, GD and GDM are approximately walking towards a "linear direction": directional Hessian characterizes the change of gradient along the update direction, and thus the gradient changes little across iterations. This agrees with the setting where we introduce effective learning rate, i.e., $\nabla f(\bw_1)\approx \nabla f(\bw_2)\approx \cdots \approx \nabla f(\bw_t)$, and thus GDM performs similarly as GD under the same effective learning rate, which explains the alignment between GD and GDM before oscillation. We summarize the above intuition as the following property.
% \citet{cohen2021gradient} regards that GD enters EoS when its sharpness reaches $\frac{2}{\eta}$. To give a simple but deep analysis of the momentum, we focus on the difference between GDM and GD in the optimization process.  Our observations(Figure \ref{fig:gd}) are:
% \begin{itemize}
%     \item For small effective learning rate where the training curves of GD and GDM coincide, both GD and GDM do not enter EoS, and both curves are smooth;
%     % \item At the turning point: {\color{red} An experiment is expected here.}
%     \item The optimizer slows down after entering the edge of stability regime. Because GDM is harder to enter EoS than GD, GDM and GD diverge after GD entering EoS.
% \end{itemize}

% \paragraph{Accelerate on Gradient Descent} Figure \ref{fig:gd} gives the result on dataset CIFAR10-5k with same effective learning rate under momentum $\mu=0.9$ and $\mu=0$. Here, we refer the optimizer with $\mu=0.0$ as GD, and optimizer with $\mu=0.9$ as GDM.
% Under small effective learning rate $\eta_{\ef}$, all the curves of GD are all most coincide with the corresponding curves of GDM. 
% In this case, both the GD and the GDM don't reach the edge of stability. Under the mild learning rate, the curves of GD are all most coincide with the corresponding curves of GDM, however, they diverge after GD reaches the edge of stability. In the edge of stability, the gradients of GD change dramatically. The GD is in edge of stability when the sharpness is larger than $\frac{2}{\eta_{\ef}}$, while the critical value is $\frac{2(1+\mu)}{\eta_{\ef}(1-\mu)}$ for GDM.



% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.4 \textwidth]{images/cifar10-5k.png}
%     \caption{\textbf{Experimental results on CIFAR10-5k dataset with different effective learning rate.} We can obtain a similar result of SGD in GD with cifar10-5k}
%     \label{fig:cifar10-5k}
% \end{figure}

% \subsection{Momentum prevents abrupt sharpening.}
% \label{subsec:momentum_abrupt_sharpening}
% There are two phenomenons that are 
% The previous section finds that before the oscillation, GDM is aligned with GD under a same effective learning rate. T


% \subsubsection{Abrupt sharpening}
% \label{subsubsc:abrupt_sharpening}

% Directional Hessian has a stronger connection to the phenomenon of EoS compared to sharpness, as the optimization process is directly influenced by the landscape in its forward direction. We explore the differences between sharpness and directional Hessian in Figure \ref{fig:gdhess}. While sharpness displays a progressive sharpening, the directional Hessian, on the other hand, demonstrates abrupt sharpening. Momentum plays a role in preventing abrupt sharpening.



% \subsubsection{SGDM is doing SGD implicitly before Abrupt Sharpening}

% We provide an further explanation of for the align-divergence pattern with the discovery of Abrupt Sharpening. To give a clearer analysis, we first rewrite the GDM to have a similar form as GD.
% \begin{proposition}
% \label{thm:mom}
% The update rule of SGDM (detail in Algorithm \ref{alg:sgd}) can be rewritten as
% \begin{gather}
% \label{lem: auxilliary}
%     \bu_1=\bw_1, \bu_{t+1}=\bu_t - \eta_{\ef} \nabla  f_{\xi_t}(\bw_t),
%     \bw_{t+1}= (1-\beta) \bu_{t+1} + \beta \bw_t.
% \end{gather}
% \end{proposition}

% \begin{remark}
% The auxiliary parameter sequence $\{\bu_t\}_{t=1}^{\infty}$ has been widely adopted in the convergence proof of momentum-based optimizers \cite{liu2020improved,wang2022does} and is used to construct potential functions, which is the key step of analysis.
% \end{remark}
% Proposition \ref{thm:mom} indicates that operating SGDM over $\{\bw_t\}_{t=1}^{\infty}$ is similar to operating SGD over $\bu_t$. The only difference is that SGDM updates $\bu_t$ with $\nabla  f_{\xi_t}(\bw_t)$ while SGD with $\nabla  f_{\xi_t}(\bu_t)$. 
\begin{proposition}
\label{prop:gdgdm}
Denote the iterations of GD as $\{\bw_t^{\GD}\}_{t=1}^{\infty}$ and those of GDM as $\{\bw_t^{\GDM}\}_{t=1}^{\infty}$. If the directional Hessians satisfy $H(\bw_s^{\GD}, \bw_{s+1}^{\GD}-\bw_{s}^{\GD})\approx 0$ and $H(\bw_s^{\GDM}, \bw_{s+1}^{\GDM}-\bw_{s}^{\GDM})\approx 0$, $\forall s\le t-1$, then we have
$
    f(\bw_t^{\GD})\approx f(\bw_t^{\GDM}).
$
\end{proposition}

\textbf{Momentum defers abrupt sharpening, and thus accelerate GD.} First of all, we show again through quadratic programming that momentum has the effect to defer abrupt sharpening.

% Below we provide a comprehensive explanation on why GDM behaves similarly as GD before GD enters EoS based on Proposition \ref{thm:mom}. Denote the parameters provided by GD as $\{\bw_t^{\GD}\}_{t=1}^{\infty}$ and those provided by SGDM as $\{\bw_t^{\GDM}\}_{t=1}^{\infty}$. According to Proposition \ref{thm:mom}, denote $\bu_1=\bw_1^{\GDM}$ and $\bu_t=\frac{\bw_{t}^{\GDM}-\beta \bw_{t-1}^{\GDM}}{1-\beta}$. We then show that $\bu_t$ is close to $\bw_t^{\GD}$ by induction. When $t=1$, the claim follows by definition. Assuming we have shown that $\bu_t\approx \bw_t^{\GD}$. Then, for the $(t+1)$-th iteration, we have
% \begin{align}
% \nonumber
%     &\bu_{t+1}- \bw_{t+1}^{\GD}=\bu_t-\bw_{t}^{\GD}-\eta_{\ef} \nabla  f(\bw^{\GDM}_t)+\eta_{\ef} \nabla  f(\bw^{\GD}_t)
%     \\
%     \label{eq: approximation}
%     \approx & -\eta_{\ef} \nabla  f(\bw^{\GDM}_t)+\eta_{\ef} \nabla  f(\bw^{\GD}_t)\approx \eta_{\ef}\nabla^2 f(\bw_t^{\GD}) (\bw_t^{\GD}-\bw_{t}^{\GDM}).
% \end{align}
% According to Proposition \ref{thm:mom}, $\bw_{t}^{\GDM}=(1-\beta)\bu_{t}+\beta \bw_{t-1}^{\GDM}= (1-\beta)\sum_{s=1}^t \beta^{t-s} \bu_s+\beta^{t-1} \bu_1 $. By induction hypothesis, we obtain $\bw_{t}^{\GDM}\approx (1-\beta)\sum_{s=1}^t \beta^{t-s} \bw_s^{\GD}+\beta^{t-1} \bw_1^{\GD} $. Therefore,
% \begin{align*}
%     \bw_t^{\GD}-\bw_t^{\GDM}\approx &\bw_t^{\GD}-\left((1-\beta)\sum_{s=1}^t \beta^{t-s} \bw_s^{\GD}+\beta^{t-1} \bw_1^{\GD}\right)
%     \\
%     =& - \eta_{\ef}\sum_{s=1}^{t-1} \beta^{t-s} \nabla f(\bw_s^{\GD})\approx - \eta_{\ef}\frac{\beta-\beta^{t}}{1-\beta} \nabla f(\bw_t^{\GD}).
% \end{align*}
% Here in the last approximate equation we use $\nabla f(\bw_{s+1}^{\GD}) -\nabla f(\bw_s^{\GD})\approx \nabla^2 f(\bw_s^{\GD})(\bw_{s+1}^{\GD}-\bw_s^{\GD}) \approx 0$ as the directional Hessian at $\bw_s^{\GD}$ along the update direction is small. Applying the above equation back to Eq. (\ref{eq: approximation}), we obtain that 
% \begin{equation*}
%      \bu_{t+1}- \bw_{t+1}^{\GD}\approx -\eta_{\ef}  \frac{\beta-\beta^{t}}{1-\beta}\nabla^2 f(\bw_t^{\GD})  \nabla f(\bw_t^{\GD})=\eta_{\ef}  \frac{\beta-\beta^{t}}{1-\beta}\nabla^2 f(\bw_t^{\GD}) (\bw_{t+1}-\bw_t)\approx 0,
% \end{equation*}
% where the last approximate equation is again due to that the directional Hessian at $\bw_t^{\GD}$ along the update direction is small. The claim is then derived by induction.

% When GD enters EoS, the directional Hessian at $\bw_t^{\GD}$ along the update direction is no longer small as abrupt sharpening happens, and the above equation fails to hold. Thus, we no longer have $\bw_{t}^{\GD}\approx \bu_t$.


% \subsubsection{Why momentum prevents abrupt sharpening}

% As the sharpness gradually increases, we find that the directional Hessian of GD experiences a sudden rise when the sharpness reaches the boundary of $\frac{2}{\eta}$. However, for GDM, this abrupt increase does not occur at this point. In the subsequent proposition, we present a mathematical analysis of the quadratic case to show the required sharpness for GD and GDM to enter the EoS.


% \begin{proposition}
% \label{prop: convergence_direction}
% Consider the quadratic programming problem $\min_{\bw \in \mathbb{R}^d} f(\bw)=\min_{\bw\in \mathbb{R}^d}\frac{1}{2} \bw^{\top} A \bw+\boldsymbol{b}^{\top}\bw+c$, where $\bA$ is a positive definite symmetric matrix. Let $\bw_t$ be the parameter given by GD at the $t$-th iteration. Let $\mathcal{A}$ be the space of eigenvectors of $\bA$ corresponding to the maximum eigenvalue of $\bA$. Then, for initialization $\bw_0\ne 0$, $\lim_{t\rightarrow \infty}\frac{\nabla f(\bw_t)}{\Vert \nabla f(\bw_t) \Vert} \in \mathcal{A} $, if and only if $\eta$ satisfies $\eta> \frac{2}{\lambda_{\max}(\bA)+\lambda_{\min} (\bA)}$.
% \end{proposition}

% \begin{proposition}
% \label{prop: convergence_direction_momentum}
% Consider the quadratic programming problem $\min_{\bw \in \mathbb{R}^d} f(\bw)=\min_{\bw\in \mathbb{R}^d} \frac{1}{2}\bw^{\top} A \bw+\boldsymbol{b}^{\top}\bw+c$, where $\bA$ is a positive definite symmetric matrix. Let $\bw_t$ be the parameter given by GDM at the $t$-th iteration. Let $\mathcal{A}$ be the space of eigenvectors of $\bA$ corresponding to the maximum eigenvalue of $\bA$. Then, for $\bw_0\in \mathbb{R}^d/\mathcal{K}$ where $\mathcal{K}$ is a zero-measure set, if $\lim_{t\rightarrow \infty}\frac{\nabla f(\bw_t)}{\Vert \nabla f(\bw_t) \Vert} \in \mathcal{A} $, then the effective learning rate $\eta_{\ef}>\max\{ \frac{2(1+\beta)}{(1-\beta)(\lambda_{\max}(\bA)+\lambda_{\min} (\bA))}, \frac{(1+\sqrt{\beta})^2}{(1-\beta)\lambda_{\max}(\bA)}\}$.
% \end{proposition}

\begin{proposition}
\label{prop: convergence_direction_momentum}
Let $f$, $\bw^*$ and  $\tilde{f}$ and $\mathcal{A}$ be defined in Proposition \ref{prop: convergence_direction_momentum}. Let $\bw_t$ be the parameter given by GDM at the $t$-th iteration.  Then, for almost everywhere $\bw_0\in \mathbb{R}^d$, $\lim_{t\rightarrow \infty}\frac{\nabla \tilde{f}(\bw_t)}{\Vert \nabla \tilde f(\bw_t) \Vert} \in \mathcal{A} $ if and only if $\lambda_{\max}(\nabla^2 f(\bw))> \frac{2(1+\beta)}{(1-\beta)\eta_{\ef}}-\lambda_{\min} (\nabla^2 f(\bw))$.
\end{proposition}
Comparing Proposition \ref{prop: convergence_direction_momentum} with Proposition \ref{prop: convergence_direction}, we observe that with a relative small $\lambda_{\min}$, the required least sharpness for abrupt sharpening of GDM is $\frac{(1+\beta)}{1-\beta}$ (which is $19$ when $\beta=0.9$) times larger than that of GD. As the sharpness progressively increases, reaching the required least sharpness of GDM takes a much longer time than reaching that of GD (an extreme case is that abrupt sharpening happens in GD but not in GDM). Meanwhile, entrance of edge of stability has been known to slow down the convergence. In \cite{ahn2022learning}, it is shown that when not entering EoS, GD converges in $\mathcal{O}(1/\eta_{\ef})$ iterations, but require $\Omega(1/\eta_{\ef}^2)$ iterations in the EoS regime. Together, we arrive at the conclusion that momentum can accelerate GD through deferring the entrance of EoS (abrupt sharpening).

% In the quadratic scenario, the abrupt sharpening happens when the gradient direction coincides with the eigenvector associated with the maximum eigenvalue of matrix $\bA$. In this case, the directional Hessian is equal to the sharpness.  If we set $\eta=\eta_{\ef}$, then the required sharpness, i.e., $\lambda_{\max}(\bA)$, for GDM  is greater than that for GD. Therefore, GDM is unlikely to go through abrupt sharpening.  

% {\color{red} Question: why entering EoS slows down the convergence? Or why GD and GDM perform similarly when not entering EoS? Do the update of GD and GDM have the same norm when the effective learning rate is small?}

% {\color{red} Question: how the EoS of GDM is defined? Maybe we can use $\frac{2}{\eta}(1+\beta)=\frac{2}{\eta_{\operatorname{ef}}}\frac{1+\beta}{1-\beta}$ in Cohen et al..}

% {\color{red} To-do list: 
% \begin{itemize}
%     \item A figure like Figure \ref{fig:elr} for GD and GDM;
%     \item An observation of the Hessian when GDM is at the turning point in the fore-mentioned figure;
%     \item A comparison of the update norm when the effective learning rate is low;
% \end{itemize}
% }


% Questions on Figure \ref{fig: gd_resnet}: why GDM starts to oscillate? It does not reach the threshold predicted in \citep{cohen2021gradient}. Why GD and GDM behaves differently before they enter EoS? 
% \paragraph{Momentum and SGD}




% \subsection{Extension to stochastic case}
% Fig \ref{fig:elr} gives the training loss at 200 epoch using SGDM under different effective learning rate with three different momentum settings. When the effective learning is small(less than 0.05), SGDM reach a similar training loss after 200 epoch. However, with the effective learning increasing, SGDM with lower $\mu$ will increase the training loss earlier.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6 \textwidth]{images/momentum.jpg}
%     \caption{Experimental results on CIFAR10 dataset with same effective learning rate under momentum $\mu=0.9$, $\mu=0.5$ and $\mu=0$}
%     \label{fig:elr}
% \end{figure}

% \textbf{Observation.}
% \begin{itemize}
%     \item The gradient norm of SGDM is larger when the effective learning rate is large. 
% \end{itemize}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9 \textwidth]{images/elr02.png}
%     \caption{}
%     \label{fig:elr}
% \end{figure}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9 \textwidth]{images/elr002.png}
%     \caption{}
%     \label{fig:elr}
% \end{figure}

\subsection{Extending the analysis to stochastic case: interplay between momentum and batch size}
\label{sc:small_batch_training}
 Over the same experiment of Sections \ref{subsc:eos_phasetransition} and \ref{sec: abrupt_effect}, we first plot the training curves of GD, GDM, and SGD with batch size $250$ and $\eta^{5000}_{\ef}=0.1$ in Figure \ref{fig:CIFAR10_5k_SGD}A. Specifically, we find that:
\begin{itemize}
    \item \textbf{Stochastic noise can also defer abrupt sharpening.} GD enters EoS during the training process, while SGD and GDM does not and remain well-aligned and throughout the training process and converges faster than GD.
\end{itemize}
Since in previous section, we have explained that entrance of EoS slows down the convergence, such an observation explains why in Figure \ref{fig:phase_transition}, reducing batch size also accelerates SGDM. Furthermore, this observation also explains why the effect of momentum is more pronounced when batch size is large since stochastic noise and momentum has an overlapping effect in preventing abrupt sharpening.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95 \textwidth]{images/CIFAR10_5k_SGD.png}
    \caption{\textbf{Stochastic noise and momentum play a duplicate role in preventing abrupt sharpening.} A: Stochastic noise can help prevent abrupt sharpening. B: When small batch size training is already employed, incorporating momentum becomes less influential.}
    \label{fig:CIFAR10_5k_SGD}
\end{figure}
Moreover, we conjecture that linear scaling law fails due to that stochastic noise can defer abrupt sharpening, and thus momentum can extend linear scaling law: the performance of large-batch SGD is worse than small-batch SGD because large-batch enters EoS while small-batch does not. When momentum is added, large-batch also does not enter EoS and the linear scaling law is extended. We show in Figure \ref{fig:CIFAR10_5k_SGD} that our conjecture is correct. 
% Figure \ref{fig:phase_transition} illustrates that raising $\mu$ and reducing batch size can speed up training when the effective learning rate exceeds a critical point. Since momentum helps prevent abrupt sharpening, we are curious to determine if small batch training serves a similar purpose.
% \begin{itemize}
%     \item \textbf{Stochastic noise can help prevent abrupt sharpening.} We perform experiments (Figure \ref{fig:CIFAR10_5k_SGD} A) using $\eta^{5000}_{\ef}=0.1$, where GD enters EoS during the training process, while SGD does not. Interestingly, SGD and GDM remain well-aligned throughout the training process. Considering these observations, we can infer that stochastic noise, much like momentum, can aid in preventing abrupt sharpening.
% \end{itemize}
% This observation corresponds with the findings in Figure \ref{fig:phase_transition} when the effective learning rate surpasses a certain threshold. Consequently, we aim to investigate the effects of utilizing both small batch training and momentum. Through the investigation of SGD with varying batch sizes (Figure \ref{fig:CIFAR10_5k_SGD} B), we observe that:

% When we set the effective learning rate as 0.5, we observe that the GDM has a similar performance as SGDM with batch size 1000, but GDM perform worse than SGD with batch size 256(Figure \ref{fig:cpsgdmom} \textit{Right}). 
% Figure \ref{fig:sgdmom} shows that SGD and Momentum have a similar effect. 


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7 \textwidth]{images/momhsgd.png}
%     \caption{\textbf{Investigating the combined effects of small batch training and momentum under $\eta^{5000}_{\ef}=0.1$.} \textit{Left:} SGD with different batch size (note that GD can be regarded as SGD with batch size 5000) \textit{Right:} SGDM with different batch size. Momentum can remove the EoS of SGD and make the curves with different batch closer with each other. }
%     \label{fig:momhsgd}
% \end{figure}



% \begin{itemize}
%     \item \textbf{The impact of momentum is more obvious when SGD has a higher tendency to enter EoS.}   SGD with varying batch sizes demonstrates distinct capabilities in averting abrupt sharpening. An optimizer tends to have a slower training speed if it is more prone to entering EoS. When momentum is incorporated into all these algorithms, the training speeds of SGD with different batch sizes become aligned. This indicates that momentum is more advantageous for large batch SGD, as it is more susceptible to entering EoS. In the case of SGD with a batch size of 250, there is minimal change observed after adding momentum.
% \end{itemize}

% These experiments provide evidence that both small batch training and momentum contribute to preventing abrupt sharpening. However, when small batch size training is already employed, incorporating momentum becomes less impactful.
% Upon incorporating momentum (Figure \ref{fig:momhsgd} \textit{Right}), SGDM with a range of batch sizes persistently evades entering EoS, leading to the alignment of their training curves. Consequently, the impact of momentum becomes more prominent when applied to the slower training velocity of SGD using larger batch sizes. 

% and learning rate linear scaling rule is not satisfied when the batch size is larger than a threshold. We find that by add momentum, we can make the threshold batch size larger. Under $\eta_{\ef}=0.5$, the optimization speed of SGD with batch size 256 is quicker than the SGD with batch size 1000(Figure \ref{fig:momhsgd} Left). However, their corresponding SGDM curves match with each other(Figure \ref{fig:momhsgd} Right). 

% \subsection{Our Answer}
% \label{subsec:answer_why}
% We associate the phase transition phenomenon with the EoS. The phase transition and entry into EoS appear to occur almost simultaneously in Figure \ref{fig:overview}. We observe that the optimizer's training speed decreases upon entering the EoS regime. Momentum can help prevent abrupt sharpening and, consequently, delay the point at which SGD enters the EoS. This effect contributes to the acceleration of the training process with momentum. Further experiments indicate that both small batch size training and momentum play a role in avoiding abrupt sharpening. As a result, the impact of momentum is less pronounced when small batch size training is already employed.


